Adapting to game trees in zero-sum imperfect information games

Imperfect information games (IIG) are games in which each player only partially observes the current game state. We study how to learn $\epsilon$-optimal strategies in a zero-sum IIG through self-play with trajectory feedback. We give a problem-independent lower bound $\widetilde{\mathcal{O}}(H(A_{\mathcal{X}}+B_{\mathcal{Y}})/\epsilon^2)$ on the required number of realizations to learn these strategies with high probability, where $H$ is the length of the game, $A_{\mathcal{X}}$ and $B_{\mathcal{Y}}$ are the total number of actions for the two players. We also propose two Follow the Regularized leader (FTRL) algorithms for this setting: Balanced FTRL which matches this lower bound, but requires the knowledge of the information set structure beforehand to define the regularization; and Adaptive FTRL which needs $\widetilde{\mathcal{O}}(H^2(A_{\mathcal{X}}+B_{\mathcal{Y}})/\epsilon^2)$ realizations without this requirement by progressively adapting the regularization to the observations.

==> main/sortofbin.tex <==
\paragraph{Theoretical results}

We first state the theoretical results on the expected regret.

\begin{theorem}\label{thm:general_bal}
    Using Algorithm \ref{al:ftrl_bal}-Tsallis, $\tsallis\in (0,1)$, $\gamma=0$ and constant learning rates $\eta_h=\pa{A_X/H}^{\tsallis-1/2}\sqrt{2\tsallis(1-\tsallis)/T}$ yields
    
    \[\pseudoregret_\mathrm{max}^T\leq \sqrt{2/(\tsallis(1-\tsallis))} \sqrt{HA_X T}\]
    
    Using Algorithm \ref{al:ftrl_bal}-Shannon, $\gamma=0$ and $\eta_h=\sqrt{{2H\log(A_X)}/\pa{A_X T}}$ yields
    
    \[\pseudoregret_\mathrm{max}^T\leq \sqrt{2\log(A_X)}\sqrt{HA_X T}\]
    
\end{theorem}

\begin{theorem}\label{thm:lb}
    (Regret lower bounds) For any height $H\geq 2$ and number of action $A_X\geq 4H$, there exists a tree structure of the information states and rewards such that
    \begin{itemize}
        \item For $T$ high enough, for any player policy, there exists some state transitions such that:
    \[\pseudoregret_\mathrm{max}^T\geq c\sqrt{HA_X T}\]
        \item (Maybe remove this one?) For any $\delta<1/8$ and $T$ high enough, for any player policy, there exists some state transitions such that, with probability at least $\delta$,
    \[\regret_\mathrm{max}^T\geq c\sqrt{HA_X T\log(1/(8\delta))}\]
    \end{itemize}
 
    (IIG lower bound) For any $H\geq 2$, $A_X,B_Y\geq 4H$ and $\delta\in(0,1/3)$, there exists a game structure and rewards such that, for any algorithm that computes an $\epsilon$-NE with probability $1-\delta$ after a fixed number $T$ of samples,
    \[T\geq cH\pa{A_X+B_Y}\log(1/\delta)/\epsilon^2\]
    
     Where $c>0$ is a fixed constant.
\end{theorem}

If the policy $\mu^\dagger \in \maxpi$ is not specified, then the regret is defined with respect to the worst one:
\[\regret^T_{\mathrm{max}}=\max_{\mu^\dagger \in \maxpi} \regret^T_{\mathrm{max}}(\mu^\dagger)\]

The expected (pseudo-)regret of the max player can also be defined with
\[\pseudoregret_{\mathrm{max}}^T=\max_{\mu^\dagger \in \maxpi} \E(\regret^T_{\mathrm{max}} (\mu^\dagger)) \]

\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|}\hline
Algorithm & Tree structure   & Varying actions & Fixed actions  \\\hline
Lower bound   & / & $\boldsymbol{\cO(\sqrt{HA_XT})}$ & $\cO(\sqrt{XAT})$  \\
(Bai and al.) & Known & / & $\tilde{\cO}(H^{3/2}\sqrt{XAT})$ \\
Algorithm \ref{al:ftrl_bal} & Known  & $\boldsymbol{\cO(\sqrt{HA_XT})}$  & $\boldsymbol{\cO(\sqrt{XAT})}$ \\
(IXOMD) & Unknown & / & $\tilde{\cO}(HX\sqrt{AT})$ \\ 
Algorithm 2 & Unknown & $\boldsymbol{\tilde{\cO}(H\sqrt{A_XT})}$ & $\boldsymbol{\tilde{\cO}(H\sqrt{XAT})}$ \\\hline

\end{tabular}
\caption{What I was picturing for the expected regret results in intro (the tilde is hard to see...), in bold the new results, of course I am bad with LaTeX, it can be improved. NE sample complexity results would be in intro text}
\end{table*}

\paragraph{Tree-like game structure and perfect recall assumption} (If we have perfect recall, we can assume WLOG a tree structure no?) We assume that the game has a tree structure: for any state $s \in \cS,$ there is a unique step $h$ and history $(s_1, a_1, b_1, \ldots, s_h = s)$ to reach~$s$. Precisely, for any policy of the players, for any realization of the game (i.e., trajectory) $(s_k',a_k',b_k')_{k\in[H]}$, conditionally to $s'_{i} = s$, it almost surely holds that $i= h$ and $(s'_1,\ldots,s'_h) = (s_1,\ldots,s_h)$. We also assume perfect recall, which means that each player remembers its past observations and actions. For example, in case of the max-player, for each information set $x \in \cX$ there is a unique history $(x_1, a_1, \ldots, x_h = x)$ up to~$x$. These assumptions require that $\cX$ can be partitioned to $H$ subsets $(\cX_h)_{h \in [H]}$ such that $x_h \in \cX_h$ is reachable only at time step $h$; otherwise there would be two different histories up to $x_h$. $\cS$, $\cY$, $\cA_\cX$ and $\cB_\cY$ can be also partitioned into $H$ subsets $(\cS_h)_{h \in [H]}$, $(\cY_h)_{h \in [H]}$, $(\cA_X^h)_{h \in [H]}$ and $(\cB_\cY^h)_{h \in [H]}$ respectively. For any $x_h\in\cX_h$, we also write $x\geq x_h$ if there exists $h'\geq h$ and an history $(x_1,a_1...,x_{h'})$ in which $x=x_{h'}$

Given the assumptions above, there exists a unique history $(s_1, a_1, b_1, \ldots, s_h=s, a_h=a, b_h=b)$ ending with $(s_h=s, a_h=a, b_h=b)$ for any state $s \in \cS_h$, max-player's action $a \in \cA_{x_h}$, and min-player's action $b \in \cB_{y_h}$. Accordingly, the probability of $s_h = s, a_h=a, b_h=b$ can be computed by $p^{\mu, \nu}_h (s, a, b) = p_{1:h} (s) \mu_{1:h} (s, a) \nu_{1:h} (s, b)$, where
\begin{align*}
  p_{1:h} (s) &:= p_0 (s_1) \textstyle\prod_{h'=1}^{h-1} p_{h'} \left(s_{h'+1} | s_{h'}, a_{h'}, b_{h'}\right),
  \\
  \mu_{1:h} (s, a) &:= \mu_{1:h} (x(s), a) := \textstyle\prod_{h'=1}^{h} \mu_{h'} \left(a_{h'} |\, x(s_{h'})\right),
  \\
  \nu_{1:h} (s, b) &:= \nu_{1:h} (y(s), b) := \textstyle\prod_{h'=1}^{h} \nu_{h'} \left(b_{h'} |\, y(s_{h'})\right).
\end{align*}
With abuse of notation, we let $\mu_{1:h-1} (s) := \mu_{1:h-1} (x(s)) := \mu_{1:h-1} (s_{h-1}, a_{h-1})$, $p^{\mu, \nu}_{1:h} (s) := p_{1:h} (s) \mu_{1:h-1} (s, a) \nu_{1:h-1} (s, b)$ and $p^{\mu, \nu}_{1:h} (x) := \sum_{s \in x(s)} p^{\mu, \nu}_{1:h} (s)$ for any information set $x \in \cX_h$. We use $\nu_{1:h-1}$ similarly.

\paragraph{Regret and Nash equilibrium}

For policies $\mu$ and $\nu$ we define the expected return (of the max-player) by $V^{\mu, \nu} := \sum_h \sum_{s_h \in \cS_h, a_h \in \cA_{x_h}, b_h \in \cB_{y_h}} p^{\mu, \nu}_{1:h} (s_h, a_h, b_h) r_h (s_h, a_h, b_h)$. For sequences of policies $\left(\mu^t\right)_{t \in [T]} \in \maxpi^T$ and $\left(\nu^t\right)_{t \in [T]} \in \minpi^T$, the regret of the max-player is defined as
\begin{align}
  \regret^T_{\mathrm{max}}:= \max_{\mu^\dagger \in \maxpi} \sum_{t=1}^T \pp{V^{\mu^\dagger, \nu^t} - V^{\mu^t, \nu^t}}.\label{eq:max regret}
\end{align}

Similarly, the same regrets can be defined for the min player using $\sum_{t=1}^T (V^{\mu^t, \nu^t} - V^{\mu^t, \nu^\dagger})$ for $\nu^\dagger \in \minpi$

There is a very clear link between minimizing the regret of both players and computing an $\epsilon$-NE. In particular, Theorem 1 of \citep{kozuno2021learning} can easily be extended to non-fixed action sets.

\begin{theorem} \label{thm:folklore}
    From $(\mu^t,\nu^t)_{t\in[T]}$ define the average profile $(\overline{\mu},\overline{\nu})$ (see ref appendix), then $(\overline{\mu},\overline{\nu})$ is an $\epsilon$-NE with
    \[\epsilon=\pa{\regret^T_{\mathrm{max}}+\regret^T_{\mathrm{min}}}/T\]
\end{theorem}

\paragraph{Loss and adversarial transitions} For any policy $\nu$ and state $s\in\Sw_h$, we can define, similarly to $p_{1:h}^{\mu,\nu}$, the adversarial transition of the max player $p_{1:h}^\nu(s):=p_{1:h}(s)\nu_{1:h-1}(s,b)$, and for $x\in \cX_h$,  $p_{1:h}^\nu(x):=\sum_{s\in x(s)} p_{1:h}^\nu(s)$. These adversarial transitions are in fact the transitions on the information states $\cX$ when playing against $\nu$, from the viewpoint of the max-player. In the rest of the article, we will call any transition on the information states an adversarial transition, not only the ones of the form $p^\nu$.

As in a bandit setting, for the max player, the losses $l^t=(l_h^t)_{h\in[H]}$ can also be defined by
\begin{align*}
    &\qquad \ell_h^t(x_h,a_h):=\\
    &\sum_{s_h\in x_h(s)}\sum_{b_h\in \cB_{y_h}}p_{1:h}(s_h)\mu_{1:h}(s_h,b_h)(1-r_h(s_h,a_h,b_h))
\end{align*}
and, defining $\mu_{1:}:=\{\mu_{1:h}\}_{h\in[H]}$ for any $\mu\in\maxpi$, along with the canonical scalar product:

\[\scal{\mu_{1:}}{l^t}:=\sum_h\sum_{(x_h,a_h)\in\cA_\cX^h}\mu_{1:h}^{}(x_h,a_h)l_h^t(x_h,a_h)\]

the regret related to $\mu^\dagger\in\maxpi$ can be rewritten:

\[\regret^T_{\mathrm{max}} (\mu^\dagger)= \max_{\mu^\dagger \in \maxpi} \sum_{t=1}^T \scal{\mu_{1:}^t-\mu_{1:}^\dagger}{l^t}\]
